Simulation Limitations of Affine Cellular Automata

Cellular automata are a famous model of computation, yet it is still a challenging task to assess the computational capacity of a given automaton; especially when it comes to showing negative results. In this paper, we focus on studying this problem via the notion of CA relative simulation. We say that automaton A is simulated by B if each space-time diagram of A can be, after suitable transformations, reproduced by B. We study affine automata - i.e., automata whose local rules are affine mappings of vector spaces. This broad class contains the well-studied cases of additive automata. The main result of this paper shows that (almost) every automaton affine over a finite field F_p can only simulate affine automata over F_p. We discuss how this general result implies, and widely surpasses, limitations of additive automata previously proved in the literature. We provide a formalization of the simulation notions into algebraic language and discuss how this opens a new path to showing negative results about the computational power of cellular automata using deeper algebraic theorems.

==> affine_cas_general.tex <==
\section{Introducing Additive and Affine Automata} \label{section:affine_introduction}

\emph{Additive automata} are a much-studied class of CAs. Studying the automata simulated by them leads naturally to a broader class of \emph{affine automata}, which we now introduce. 

\begin{defn} [affine CA, additive CA]
    Let $\F$ be a finite field, $V$ a finite-dimensional vector space over $\F$, and let $\A = (V^\Z, F)$ be a CA with local algebra $(V, f)_r$. We say that $\AA$ (or $\A$) is \emph{affine over $\F$} if $f: V^{2r+1} \rightarrow V$ is an affine mapping between vector spaces over $\F$. In such a case, we can write $f$ in the following form:
    \begin{align} \label{def:affine_f}
        f(\xx_{-r}, \ldots, \xx_r) = f_{-r}(\xx_{-r}) + \cdots + f_r(\xx_r) + \cc,
    \end{align}
    where $f_i: V \rightarrow V$ is a linear mapping for each $-r \leq i \leq r$ and $\cc \in V$ is a constant vector. The mapping $f_i$ is called the \emph{$i$-th component of $f$}. The class of all local algebras isomorphic to some affine local algebra over $\F$ with radius $r$ is denoted as $\AFF^\F_r$.

    In the special case when $f: V^{2r+1} \rightarrow V$ is a linear mapping between vector spaces over $\F$, we say that $\AA$ (or $\A$) is \emph{additive over $\F$}. In such a case, we can write $f$ as in (\ref{def:affine_f}) with $\cc = \vo$. We denote the class of all local algebras isomorphic to some local algebra additive over $\F$ with radius $r$ as $\ADD^\F_r$. We say that $\AA$ is \emph{canonical additive (or affine)} if it is additive (or affine) over $\F_p$ for some prime $p$ and $V = \F_p$. 
\end{defn}

\begin{ex}
    Let $(\F_2^\Z, F)$ be the elementary CA 150 with local algebra $\AA = (\F_2, f)_1$ where $f: \F_2^3 \rightarrow \F_2$ is defined as $f(x,y,z)=x+y+z \bmod 2$. Then, $\AA$ is a CA additive over $\F_2$; in fact, it is canonical additive.
\end{ex}

Automata additive over finite fields of the form $\F_p$, $p$ prime, have been widely studied. In fact, they form one of the few classes of cellular automata that are amenable to algebraic analysis which yields rigorous results about their global dynamics. To name a few important results not directly related to CA simulation, the properties of the additive CAs' global dynamics have been carefully analysed in the seminal work \cite{algebraic_properties_of_ca} and consequently in \cite{exact_results_for_determinstic_cas, linear_cas_and_recurring_sequences, self_similarity_of_linear_cas, linear_cas_finite_automata_pascals_triangle}. We remark that additive automata are sometimes also called \emph{linear} in the literature.

The class of affine automata is a natural generalization of additive CAs that occurs when we study sub-automata of additive CAs. As shown further in the next section, it is the case that sub-automata of additive CAs need not be additive but are in general affine. To get acquainted with the two notions, we start with a simple lemma and an example.

\begin{lemma} \label{obs:additive_idempotent}
    Let $\F$ be a finite field and $r \in \N$. Let $\AA = (V, f)_r$ be such that $\AA \in \AFF^\F_r$. Then, $\AA \in \ADD^\F_r$ if and only if there exists an idempotent element of $f$; i.e., there exists $\vv \in V$ such that $f(\vv, \ldots, \vv)=\vv$.
\end{lemma}
\begin{proof}
    Each additive CA has $\vo$ as an idempotent element. In the other direction, let $\AA = (V, f)_r$ be such that $\AA \in \AFF^\F_r$, and suppose that $\vv \in V$ is an idempotent of $f$. Let $f_{-r}, \ldots, f_r$ be the components of $f$. We define the bijection $\varphi: V \rightarrow V$ as $\varphi(\vv + \xx) = \xx$ for every $\xx \in V$. Next, we define $g:V^{2r+1} \rightarrow V$ as $g(\xx_{-r}, \ldots, \xx_r) \coloneqq \sum_{i=-r}^r f_i(\xx_i)$. Then, the CA with local algebra $(V, g)_r$ is additive, and it is straightforward to verify that $(V, f)_r \cong (V, g)_r$ via $\varphi$; indeed, for any $\xx_{-r}, \ldots, \xx_r$ we have:
    \begin{align*}
        \varphi\left(f(\xx_{-r}+\vv, \ldots, \xx_r+\vv)\right) &= \varphi\bigl(f(\vv, \ldots, \vv)+\sum_{i=-r}^r f_i(\xx_i)\bigr) = \sum_{i=-r}^r f_i(\xx_i)=\\ 
        &= \sum_{i=-r}^r f_i(\varphi(\xx_i+\vv))=g\left(\varphi(\xx_{-r}+\vv), \ldots, \varphi(\xx_{r}+\vv))\right). \qedhere
    \end{align*} 
\end{proof}


\begin{ex}
    $\ADD^{\F_2}_1 \subsetneq \AFF^{\F_2}_1$. An example of an affine CA that is not isomorphic to any additive one is the elementary CA 105 with local algebra $(\F_2, f)_1$ where $f(x,y,z)=(x+y+z+1) \bmod 2$ for any $x,y,z \in \F_2$. It is clear that neither 0 nor 1 are idempotent elements of $f$.
\end{ex}



Many of the results presented in this paper hold for affine CAs with at least two components that are bijections. A special case of such rules are the \emph{left- or right-permutive CAs} that are well studied in the literature \cite{topological_dynamics_of_cellular_automata}. Below, we define the left- and right-permutivity for affine automata in a slightly more general way compared to the classical definition to account for the fact that we only study cellular automata with a symmetrical neighbourhood given by a particular radius.


\begin{defn} \label{def:bijectivity}
Let $\AA=(V,f)_r$ be an affine local algebra of a CA with radius $r$ whose local rule $f$ has components $f_{-r}, \ldots, f_r$. We say that $\AA$ satisfies the \emph{bijective condition} if at least two of the components are bijections. 
We say that $\AA$ is \emph{left-permutive, witnessed by $i$,} if there exists $-r \leq i \leq r$ such that $f_i$ is a bijection and $f_k$ is the constant $\vo$ mapping for all $k < i$. Similarly, $\AA$ is \emph{right-permutive, witnessed by $j$,} if there exists $-r \leq j \leq r$ such that $f_j$ is a bijection and $f_k$ is the constant $\vo$ mapping for all $k > j$.

We write that $\AA \in \AFF^\F_{r;i,j}$ if $\AA \in \AFF^\F_{r}$ and at the same time $\AA$ is left-permutive witnessed by $i$ and right-permutive witnessed by $j$, $i < j$. Clearly, all such algebras satisfy the bijective condition. Analogously, we define the subclass $\ADD^\F_{r;i,j}$.
\end{defn}

Now we can state the main result of this paper that we prove in Section \ref{section:affine_limitations}:

\begin{thm}\label{thm:main_result}
    Let $p$ be a prime, $r \in \N$, and $-r \leq i < j \leq r$. Let $\AA$, $\BB$ be local algebras of cellular automata with radius $r$ such that $\BB \in \AFF^{\F_p}_{r;i,j}$. If $\AA \preceq \BB$, then $\AA \in \AFF^{\F_p}_{r;i,j}$.
\end{thm}


\subsection{Related Work on CA Simulation} \label{subsection:related_work}


In their seminal work \cite{inducing_order_on_ca_by_grouping}, Mazoyer and Rapaport study the properties of a strongly related notion of CA simulation based on iterative powers and sub-automata. In \cite{additive_cas_over_Zp_bottom}, they specifically focus on showing that a particular class of canonical additive CAs is limited in terms of what it can simulate. Subsequently, their work was continued in the collaboration \cite{bulking1}, where the authors introduce a generalized version of the iterative powers of CAs that we denote here by $\widetilde{\Xi}$ for clarity. Informally, $\widetilde{\Xi}$ allows for much more general geometrical transformations of the CA space-time diagrams. Whereas $\Xi$ is based on grouping together blocks of consecutive ``cells'' via the operators $o_n$, $\widetilde{\Xi}$ allows for groupings of much more general patterns, as well as, e.g., shifts of the CA's configuration space. In their subsequent work \cite{bulking2}, the same authors introduce various notions of CA simulation; the most general one is roughly defined below. 


\begin{defn} [CA Simulation: Delorme, Mazoyer, Ollinger, Theyssier \cite{bulking2}]
    Let $\A$ and $\B$ be two 1D CAs both with radius $r \in \N$. For their local algebras, we write $\AA \preceq_\mathrm{m} \BB$ if $\widetilde{\Xi}(\AA) \cap \HHH\SSS\widetilde{\Xi}(\BB) \neq \emptyset$.
\end{defn}

Both lines of work (\cite{inducing_order_on_ca_by_grouping, additive_cas_over_Zp_bottom} and \cite{bulking1, bulking2}) analyse various important properties of the different CA simulations. This includes studying the simulation limitations of a special family of additive automata, namely those with local algebras of the form $\ZC_p = (\F_p, f)_1$ where $f(x, y, z)=(x+y+z) \bmod p$. Their negative result is that whenever $p \neq q$, one has $\ZC_p \npreceq_\mathrm{m} \ZC_q$. The authors use two observations:
\begin{enumerate}
    \item Let $\AA$, $\BB$ be local algebras of CAs with radius $r$. Then, $\widetilde{\Xi}(\AA) \cap \HHH\SSS\widetilde{\Xi}(\BB) \neq \emptyset$ if and only if $\widetilde{\Xi}(\AA) \cap \HHH\SSS\Xi(\BB) \neq \emptyset$.
    \item Let $\AA$ be a local algebra of a CA with $p$ states. Then the algebras in $\widetilde{\Xi}(\AA)$ have $p^k$ states, $k \geq1$.
\end{enumerate}
Given the observations, the authors reduce the problem of showing $\ZC_p \npreceq_\mathrm{m} \ZC_q$ for $p \neq q$ to proving that any algebra in $\HHH\SSS\Xi(\ZC_q)$ has $q^l$ elements for some $l \geq 0$. Assuming this extra piece of knowledge, which we deduce below as a corollary of our work, comparing the sizes of algebras in $\HHH\SSS\Xi(\ZC_q)$ and in $\widetilde{\Xi}(\ZC_p)$ already implies the negative result, as $p^k \ne q^l$ for $k\ge 1$, $l \geq 0$.

The crucial information about possible sizes of algebras in $\HHH\SSS\Xi(\ZC_q)$ follows immediately from our results. (This is not surprising, since Theorem \ref{thm:main_result} provides a lot of information about the structure of these algebras.) Indeed: For every prime $q$, clearly $\ZC_q \in \ADD^{\F_q}_{1;-1,1}$. By Theorem \ref{thm:main_result}, any local algebra in $\HHH\SSS\Xi(\ZC_q)$ belongs to $\AFF^{\F_q}_{1;-1,1}$; therefore it has an underlying structure of a vector space over $\F_q$ and hence, it has $q^l$ elements.

%Below, we briefly discuss how Theorem \ref{thm:main_result} immediately implies that $\ZC_p \npreceq_\mathrm{m} \ZC_q$ for $p \neq q$.
%
%For every prime $q$, clearly $\ZC_q \in \ADD^{\F_q}_{1;-1,1}$. Let $p, q$ be distinct primes. Theorem \ref{thm:main_result} implies that $\HHH\SSS\Xi(\ZC_q) \subseteq \AFF^{\F_q}_{1;-1,1}$. Thus, any local algebra in $\HHH\SSS\Xi(\ZC_q)$ has $q^l$ elements, $l \geq 0$. In contrast, all local algebras from $\widetilde{\Xi}(\ZC_p)$ have $p^k$ elements, $k \geq 1$. Thus, just comparing the algebra sizes implies that $\widetilde{\Xi}(\ZC_p) \cap \HHH\SSS\Xi(\ZC_q) = \emptyset$, and thus $\ZC_p \npreceq_\mathrm{m} \ZC_q$.





